A matrix analysis approach to discrete comparison principles for nonmonotone PDE

We consider a linear algebra approach to establishing a discrete comparison principle for a nonmonotone class of quasilinear elliptic partial differential equations. In the absence of a lower order term, we require local conditions on the mesh to establish the comparison principle and uniqueness of the piecewise linear finite element solution. We consider the assembled matrix corresponding to the linearized problem satisfied by the difference of two solutions to the nonlinear problem. Monotonicity of the assembled matrix establishes a maximum principle for the linear problem and a comparison principle for the nonlinear problem. The matrix analysis approach to the discrete comparison principle yields sharper constants and more relaxed mesh conditions than does the argument by contradiction used in previous work.

==> makefile <==
#! make
##############################################################################
# Purpose: MCP (Mathematical and Computational Physics Group) paper makefile.
#
# Notes:   This makefile is used by the MCP group (Michael Holst's Research 
#          Group in the Mathematics and Physics Departments at UC San Diego)
#          to build latex papers using the fairly simple combination of 
#          pdflatex, amstex/amslatex, and pdf/png images.
#
# Targets: The makefile will auto-generate the following based on the
#          requested make target:
#
#            Main Targets:
#
#              pdfth   --> ${TARGET}.pdf via pdflatex
#              pdf     --> ${TARGET}.pdf via pdflatex + thumbpdf
#              dvi     --> ${TARGET}.dvi via latex
#              dvip    --> ${TARGET}.dvi|ps|pdf via latex + dvips + ps2pdf
#
#            Auxilliary Targets:
#
#              arx     --> zarxiv.tar.gz (gzipped tarball for arXiv)
#              clean   --> rm -f *.aux, *.dvi, etc
#              rclean  --> clean + rm *.ps *.bbl (careful!)
#              rrclean --> rclean + rm m.pdf mm.pdf ${TARGET}.pdf (careful!)
#
# Author:  Michael Holst
# Date:    Sat Dec 19 22:23:18 PST 2009
##############################################################################

default: pdf

TARGET=PoZh17d

ARXIV_DIR=zarxiv
ARXIV_FILES=${TARGET}.tex ${TARGET}.bbl \

LATEX=latex
PDFLATEX=pdflatex
#PDFLATEX=pdflatex --shell-escape
BIBTEX=bibtex
#BIBTEX=./zbibtex

all : pdf arx

dvi :
	make clean
	${LATEX} ${TARGET}.tex
	-${BIBTEX} ${TARGET}
	${LATEX} ${TARGET}.tex
	${LATEX} ${TARGET}.tex
	-cp -f ${TARGET}.dvi mm.dvi

dvip : dvi
	dvips -N0 -P pdf -t letter -o ${TARGET}.ps mm.dvi
	ps2pdf ${TARGET}.ps
	-cp -f ${TARGET}.pdf mm.pdf

pdf :
	make clean
	${PDFLATEX} ${TARGET}
	-${BIBTEX} ${TARGET}
	${PDFLATEX} ${TARGET}
	${PDFLATEX} ${TARGET}
	-cp -f ${TARGET}.pdf mm.pdf

pdfth : pdf
	thumbpdf ${TARGET}
	${PDFLATEX} ${TARGET}
	rm -f thumb*.png
	-cp -f ${TARGET}.pdf mm.pdf

arx : ${TARGET}.bbl
	./makex ${ARXIV_DIR} ${ARXIV_FILES}

clean :
	rm -f *.aux *.dvi *.log *.lof *.lot *.toc *.blg *.idx *.out *.tpt

rclean :
	make clean
	rm -f *.ps *.bbl

rrclean :
	make rclean
	rm -f m.pdf mm.pdf ${TARGET}.pdf
	rm -rf ${ARXIV_DIR}


